Bottom-Up Synthesis of Knowledge-Grounded Task-Oriented Dialogues with Iteratively Self-Refined Prompts

Training conversational question-answering (QA) systems requires a substantial amount of in-domain data, which is often scarce in practice. A common solution to this challenge is to generate synthetic data. Traditional methods typically follow a top-down approach, where a large language model (LLM) generates multi-turn dialogues from a broad prompt. Although this method produces coherent conversations, it offers limited fine-grained control over the content and is susceptible to hallucinations. We introduce a bottom-up conversation synthesis approach, where QA pairs are generated first and then combined into a coherent dialogue. This method offers greater control and precision by dividing the process into two distinct steps, allowing refined instructions and validations to be handled separately. Additionally, this structure allows the use of non-local models in stages that do not involve proprietary knowledge, enhancing the overall quality of the generated data. Both human and automated evaluations demonstrate that our approach produces more realistic and higher-quality dialogues compared to top-down methods.

==> Content/Introduction_old.tex <==

\section{Introduction and Related Work}
% Motivation: https://waitwhile.com/blog/virtual-personal-shopping-retail/

% \begin{figure}[h!]
% \centering
%   \includegraphics[width=\columnwidth]{Figs/dial.pdf}
%   \caption{An example dialogue from our Shopping Companion Dataset (SCD)}
%   \label{fig:dial}
% \end{figure}


% Consumer shopping is an inherently social activity in which companionship not only leads to improved customer experiences but also a higher likelihood of making a purchase ~\citep{borges2010does,granbois1968improving}. In physical-world commercial settings, many companies identify customer satisfaction as a critical factor to optimize for and stress the importance of improving ``customer-employee'' relationships~\cite {roozen2019importance}. With e-commerce growing its share of all commercial transactions year-over-year (with a particularly large surge after the onset of the COVID-19 pandemic;~\citet{bauer2023effects}), it is crucial that e-commerce companies learn to adopt these principles of companionship to emulate the brick-and-mortar shopping experience.

% Personalization is integral component of the consumer shopping experience.  --- see statistic from article above

% Shopping in real life is improved by good customer service: https://www.highspeedtraining.co.uk/hub/good-customer-service-retail/




% E-commerce should not be any different
Conversational assistants for the e-commerce domain~\cite{balakrishnan2024conversational, bernard2023mg,chiu2022salesbot} have become popular because of their potential positive effects on the shopping experience \cite{borges2010does,granbois1968improving}. Typically, these assistants streamline various customer service processes, from answering common queries to guiding users through purchasing decisions. Despite their growing utility, the development and improvement of conversational assistants are hampered by privacy and safety concerns that limit access to real user data~\cite{shi2022selective,carlini2019secret, lau2018alexa}. This limitation poses a significant challenge, as these models require vast amounts of high-quality, in-distribution data to function effectively.

% Conversational assistants are becoming increasingly integral to the e-commerce landscape, significantly enhancing customer interactions and providing personalized support. 
% Typically, these assistants streamline various customer service processes, from answering common queries to guiding users through purchasing decisions. Despite their growing utility, the development and improvement of conversational assistants are hampered by privacy and safety concerns that limit access to real user data. This limitation poses a significant challenge, as these models are fundamentally data-driven and require vast amounts of high-quality data to function effectively.

% \begin{figure}[t]
% \centering
%   \includegraphics[width=0.7\columnwidth]{example-image-golden}
%   \caption{a comparison between normal top-down dialogue synthesis and our bottom-up synthesis}
%   \label{fig:experiments}
% \end{figure}

Addressing this challenge of limited in-distribution data, researchers have developed more sample-efficient training methods for generative models. These methods include dialogue-specific pre-training objectives \cite{he2022galaxy}, improved domain adaptation through embedding learning \cite{zhao2018zero} and meta-learning \cite{qian2019domain}, or reinforcement learning approaches for task-oriented dialogues \cite{chen2024learning}.
However, such training methods are either computationally expensive or still rely on having sufficient cross-domain or in-domain seed data.

An increasingly popular strategy is to leverage large language models (LLMs) to 
synthesize dialogue data~\cite{chen-etal-2023-places,kim-etal-2023-soda}. Such methodologies for generating data in the conversational question-answering domain predominantly adopt \textbf{a top-down approach}: dialogues are crafted starting from a high-level outline and then fleshed out into detailed interactions. While this approach can produce coherent dialogues, it often lacks the granularity necessary for creating nuanced and realistic conversational datasets~\cite{zhou2024real, hayati2023far}.

To address these challenges, we propose a novel approach to constructing dialogue datasets from the \textbf{bottom up}. Our approach begins with generating high-quality question-answer pairs, which serve as the foundational building blocks for complex dialogues. Upon establishing a robust set of question-answer pairs, we connect these pairs into a coherent and contextually appropriate dialogue.

A key component of our methodology is the introduction of Self-Prompt Refinement Editing (SPREE). SPREE iteratively improves prompt quality by leveraging LLMs to evaluate and refine the generated questions. This self-refinement process ensures that the prompts are continually enhanced, producing more accurate and relevant question-answer pairs.

We employ human annotators and LLM agents to validate the quality of our synthetic dialogues. Our experimental results demonstrate that the use of iteratively self-refined prompts leads to realistic question generation, and the bottom-up synthesis framework effectively ensures the quality of the synthesized dialogues.

% This method aims to offer greater control and precision in data generation, thereby improving the quality and reliability of the resulting dialogues. 

% \looseness-1
% In this work, we address these challenges through three main contributions. 1) We propose a novel prompt-based data synthesis approach called Iterative \textit{S}elf-refinement for \textit{Pr}ompt \textit{E}m\textit{e}nding (SPREE). SPREE iteratively self-refines prompt quality for data generation by using LLM-based evaluation on synthetic question-answering pairings. 2) We apply SPREE to the e-commerce domain and then perform bottom-up dialogue generation by conditioning on these question-pairings to ensure contextual coherence and factuality. The result is our new Shopping Companion Dataset (SCD), which will be released with a permissive open-source license. We propose six guiding principles for future researchers to follow for high-quality dialogue data synthesis. 3) We provide a comprehensive evaluation of our synthesized dialogues using human annotators and LLM-based evaluation along the criteria of standards of coherence, factualness, and realism. Our experimental results demonstrate that SPREE leads to realistic question generation for grounding and that high dialogue quality is maintained despite the bottom-up nature of conversation synthesis.
% \textbf{contribution}:
% \begin{itemize}
%     \item self-refinement for prompt editing. we apply this method to generate realistic questions. we propose automatic agent evaluation to provide feedback for self-refinement
%     \item bottom-up dialogue synthesis for factualness. we also propose six principles for synthesis.
%     \item comprehensive evaluation 
% \end{itemize} 

% To address these challenges, we propose a novel approach to constructing dialogue datasets from the bottom up. This method aims to offer greater control and precision in data generation, thereby improving the quality and reliability of the resulting dialogues. Our approach begins with the generation of high-quality question-answer pairs, which serve as the foundational building blocks for more complex dialogues.

% A key component of our methodology is the introduction of Self-Prompt Refinement Editing (SPREE). SPREE iteratively improves prompt quality by leveraging LLMs to evaluate and refine the generated questions automatically. This self-refinement process ensures that the prompts are continually enhanced, leading to the production of more accurate and relevant question-answer pairs.

% Once a robust set of question-answer pairs is established, we construct the dialogue data by connecting these pairs in a coherent and contextually appropriate manner. To ensure the synthesized dialogues are coherent, factual, and realistic, we adhere to six guiding principles for dialogue synthesis. These principles are designed to maintain the natural flow of conversation and uphold the integrity of the information being exchanged.

% To validate the quality of our synthesized dialogues, we employ both human annotators and LLM agents for evaluation. This dual evaluation process provides a comprehensive assessment of the dialogues, ensuring that they meet the desired standards of coherence, factualness, and realism. Our experimental results demonstrate that the use of iteratively self-refined prompts leads to realistic question generation, and the bottom-up synthesis framework effectively ensures the quality of the synthesized dialogues.
% \textbf{contribution}:
% \begin{itemize}
%     \item self-refinement for prompt editing. we apply this method to generate realistic questions. we propose automatic agent evaluation to provide feedback for self-refinement
%     \item bottom-up dialogue synthesis for factualness. we also propose six principles for synthesis.
%     \item comprehensive evaluation 
% \end{itemize}
% In conclusion, our proposed approach to constructing dialogue datasets from the bottom up represents a significant advancement in the field of conversational AI. By focusing on the generation of high-quality question-answer pairs and employing iterative self-refinement, we can create more controlled and precise dialogue datasets. This, in turn, enhances the overall effectiveness and reliability of conversational assistants in e-commerce and beyond.

==> Content/Related_works.tex <==
\section{Related Work}
\label{sec:related_work}

\noindent \textbf{Dialogue Generation With Limited Data.}
A common approach to dealing with limited amounts of in-distribution dialogue data is developing sample-efficient methods for training generation models. \citet{he2022galaxy} developed a dialogue-specific pre-trained model using a semi-supervised objective aligned with dialogue policy learning. Another line of work examines improved domain adaptation, e.g. by proposing an approach for learning a cross-domain embedding space for generalizable dialogue generation models~\cite{zhao2018zero} or using meta-learning to enable efficient downstream domain adaptation~\cite{qian2019domain}. Recent work similarly examined domain adaptation in goal-oriented dialogues by proposing a quasi-online reinforcement learning approach based on contrastive dialogue action pairings~\cite{chen2024learning}.
However, such training methods often are computationally expensive, rely on sufficient out-of-domain data for cross-domain generalization, or depend on in-domain seed data.

A common solution in the regime of no downstream data is to directly synthesize large amounts of conversational data. \citet{chen-etal-2023-places} used expert-written in-context examples to steer LLMs to synthesize social conversations. Similarly, \citet{kim-etal-2023-soda} prompted LLMs conditioned on contextual knowledge from a knowledge graph to synthesize a dataset consisting of millions of open-domain dialogues. Other work focused specifically on question-answering contexts, synthesizing question pairings conditioned on ground-truth conversations~\cite{hwang2022conversational, gu2021chaincqg, do2022cohs}, or conditioned on questions' answers themselves~\cite{gao2019interconnected, wang2023tagnet}. 


\noindent \textbf{Prompt Optimization.}
Much work on LLMs has investigated prompt optimization for improving task performances. These studies propose approaches such as gradient-gudied search~\cite{shin2020autoprompt}, task-specific pseudo-demonstration scoring~\cite{wan2023universal}, training prompt re-writers~\cite{li2024learning}, performance optimization using prompt mixtures~\cite{wang2024one}, and self-refinement for improved task formance~\cite{madaan2024self}. Other work looks at prompt refinement for precise expressions in image generation based on automatic evaluation~\cite{wang2023reprompt}. 


\looseness-1
Here, we tackle the setting in which there is no in-distribution conversational question-answering data. Rather than synthesizing these dialogues in a top-down approach or conditioned on a set of ground truth answers, we iteratively refine a set of synthetic question-answer pairings.
